Counterfactual Fairness in Mortgage Lending via Matching and Randomization

Unfairness in mortgage lending has created generational inequality among racial and ethnic groups in the US. Many studies address this problem, but most existing work focuses on correlation-based techniques. In our work, we use the framework of counterfactual fairness to train fair machine learning models. We propose a new causal graph for the variables available in the Home Mortgage Disclosure Act (HMDA) data. We use a matching-based approach instead of the latent variable modeling approach, because the former approach does not rely on any modeling assumptions. Furthermore, matching provides us with counterfactual pairs in which the race variable is isolated. We first demonstrate the unfairness in mortgage approval and interest rates between African-American and non-Hispanic White sub-populations. Then, we show that having balanced data using matching does not guarantee perfect counterfactual fairness of the machine learning models.

==> discuss.tex <==
\textbf{Limitations of Counterfactual Fairness}
We need to carefully list all of the limitations of the approach. 
\begin{itemize}
    \item It does not account for the fact that a smaller fraction of black population apply for mortgage.
    \item \citet{lee2021algorithmic} argue that, based on financial market dynamics, simply making fair predictions does not address the issue of fairness.
    \item An approach that helps solve the problem, rather than just identifies it?....I think we need to explain how we have and have not addressed the concerns articulated by Lee and Floridi: 

"Existing approaches to fairness impose an absolute mathematical condition, whether comparing outcomes between groups, similar individuals, or group error rates. They do not account for bias embedded in the data. While these metrics are useful in quantifying the disparity, they are agnostic to the context. They have limited interpretability of outcomes specific to each use case and are challenging to set up when the proxy for outcome is intertwined with the proxy for race. Moreover, they only focus on the risk for the minority group without an eye to the potential benefits of the algorithm.

Rather than evaluating fairness against an absolute target (e.g. outcome disparity of 0), a decision-maker may consider fairness as a relative notion, shifting the focus from the quantification of unfairness against a formula to how the algorithm performs in comparison to other possible algorithms. If the goal is to select the best possible algorithm, the fairness metrics may not fully embody what is “best.” In reality, a decision-maker has several competing objectives.

While it may be impossible to remove all bias, it is possible to build an algorithm that is fairer and more accurate than the alternative. A new approach is required that builds on the previous fairness definitions but leverages the context-dependency of the data available and the relational nature of whether a decision is fair. This would provide more holistic and tangible information to the lender."
\end{itemize}
